Generalizing Event-Based Motion Deblurring in Real-World Scenarios

Event-based motion deblurring has shown promising results by exploiting low-latency events. However, current approaches are limited in their practical usage, as they assume the same spatial resolution of inputs and specific blurriness distributions. This work addresses these limitations and aims to generalize the performance of event-based deblurring in real-world scenarios. We propose a scale-aware network that allows flexible input spatial scales and enables learning from different temporal scales of motion blur. A two-stage self-supervised learning scheme is then developed to fit real-world data distribution. By utilizing the relativity of blurriness, our approach efficiently ensures the restored brightness and structure of latent images and further generalizes deblurring performance to handle varying spatial and temporal scales of motion blur in a self-distillation manner. Our method is extensively evaluated, demonstrating remarkable performance, and we also introduce a real-world dataset consisting of multi-scale blurry frames and events to facilitate research in event-based deblurring.

==> figs/main/fig-Ablation.tex <==
\def\scc{(-0.65,-0.5)}
\def\imgWidth{0.158\linewidth} %子图大小

\begin{figure}[t]
	\centering
	\begin{subfigure}{\linewidth}
	% \begin{overpic}[width=\imgWidth]{imgs/main/Ablation/Blur-1x.png}
 %    \put(1,4){\footnotesize \textcolor{white}{\bf LR blur}}
 %    \end{overpic}
    \begin{overpic}[width=\imgWidth]{imgs/main/Ablation/model1-1x.png}
    \put(1,4){\footnotesize \textcolor{white}{\bf \#1}}
    \end{overpic}
    \begin{overpic}[width=\imgWidth]{imgs/main/Ablation/model2-1x.png}
    \put(1,4){\footnotesize \textcolor{white}{\bf \#2}}
    \end{overpic}
    \begin{overpic}[width=\imgWidth]{imgs/main/Ablation/model3-1x.png}
    \put(1,4){\footnotesize \textcolor{white}{\bf \#3}}
    \end{overpic}
    \begin{overpic}[width=\imgWidth]{imgs/main/Ablation/model5-1x.png}
    \put(1,4){\footnotesize \textcolor{white}{\bf \#4}}
    \end{overpic}
    \begin{overpic}[width=\imgWidth]{imgs/main/Ablation/model4-1x.png}
    \put(1,4){\footnotesize \textcolor{white}{\bf \#5}}
    \end{overpic}
    \begin{overpic}[width=\imgWidth]{imgs/main/Ablation/model6-1x.png}
    \put(1,4){\footnotesize \textcolor{white}{\bf \#6}}
    \end{overpic}
    \\
	% \begin{overpic}[width=\imgWidth]{imgs/main/Ablation/Blur-4x.png}
 %    \put(1,4){\footnotesize \textcolor{white}{\bf HR blur}}
 %    \end{overpic}
    \begin{overpic}[width=\imgWidth]{imgs/main/Ablation/model1-4x.png}
    \put(1,4){\footnotesize \textcolor{white}{\bf \#1}}
    \end{overpic}
    \begin{overpic}[width=\imgWidth]{imgs/main/Ablation/model2-4x.png}
    \put(1,4){\footnotesize \textcolor{white}{\bf \#2}}
    \end{overpic}
    \begin{overpic}[width=\imgWidth]{imgs/main/Ablation/model3-4x.png}
    \put(1,4){\footnotesize \textcolor{white}{\bf \#3}}
    \end{overpic}
    \begin{overpic}[width=\imgWidth]{imgs/main/Ablation/model5-4x.png}
    \put(1,4){\footnotesize \textcolor{white}{\bf \#4}}
    \end{overpic}
    \begin{overpic}[width=\imgWidth]{imgs/main/Ablation/model4-4x.png}
    \put(1,4){\footnotesize \textcolor{white}{\bf \#5}}
    \end{overpic}
    \begin{overpic}[width=\imgWidth]{imgs/main/Ablation/model6-4x.png}
    \put(1,4){\footnotesize \textcolor{white}{\bf \#6}}
    \end{overpic}
	\caption{\rmfamily \fontsize{8pt}{0} Qualitative comparisons}
	\label{fig:ablation-quali-res}
	\end{subfigure}
	\begin{subfigure}{0.48\linewidth}
	    \includegraphics[width=\linewidth]{imgs/main/Ablation/fig-temporal-curve.png}
	    \caption{\rmfamily \fontsize{8pt}{0} Temporal comparisons}
	    \label{fig:ablation-temporal-curve}
	\end{subfigure}
	\begin{subfigure}{0.48\linewidth}
	    \includegraphics[width=\linewidth]{imgs/main/Ablation/fig-spatial-curve.png}
	    \caption{\rmfamily \fontsize{8pt}{0} Spatial comparisons}
	    \label{fig:ablation-spatial-curve}
	\end{subfigure}
	% \vspace{-.75em}
	\caption{Results of different models in Tab.~\ref{tab:ablation} on the Ev-REDS dataset. (a) Qualitative comparisons under $\mathcal{R}(B_T,\mathcal{E}_{\mathcal{T}})=1$ (top row) and $\mathcal{R}(B_T,\mathcal{E}_{\mathcal{T}})=4$ (bottom row). (b, c) Comparisons of models using one-stage and two-stage training, \ie, model \#3 and \#6, under different temporal and spatial scales of motion blur.  $\#S$ denotes the number of sharp images used to synthesize one blurry frame, and larger $\#S$ indicates more blurred frames.
	}
	\label{fig:ablation}
        % \vspace{-1em}
\end{figure}

==> figs/main/fig-Ev-REDS.tex <==
\def\scc{(-1.38,-0.75)}
\def\boxloc{(-1.65,-0.2)}
\def\imgWidth{0.162\textwidth} %子图大小

\def\ssizz{1cm} %框大小
\def\ssmag{3}
\def\smallboxloc{(-0.8,0.38)} % 绿色小方框位置
\def\largeboxloc{(1.37, 0.4)} % 绿色大方框位置

\begin{figure*}[t]
	\centering
	\tikzstyle{img} = [rectangle, minimum width=\imgWidth, draw=white]
% 	\rotatebox[origin=c]{90}{\centering \scriptsize{hahahahhah}}
	\begin{tikzpicture}	[spy using outlines={green,magnification=\ssmag,size=\ssizz},inner sep=0]
	   % \node [anchor=west,font=\fontsize{6}{6}\selectfont] at \boxloc {\rotatebox{90}{LR frames \& events}};
        \node [align=center, img] {\includegraphics[width=\imgWidth]{imgs/main/Ev-REDS/Blur-1x.png}};         \spy on \smallboxloc in node [left] at \largeboxloc;
        \node [anchor=west,font=\fontsize{8}{8}\selectfont] at \scc {\textcolor{white}{\bf  LR blur}};
	\end{tikzpicture}
	\begin{tikzpicture}	[spy using outlines={green,magnification=\ssmag,size=\ssizz},inner sep=0]
        \node [align=center, img] {\includegraphics[width=\imgWidth]{imgs/main/Ev-REDS/GT-1x.png}};         \spy on \smallboxloc in node [left] at \largeboxloc;
        \node [anchor=west,font=\fontsize{8}{8}\selectfont] at \scc {\textcolor{white}{\bf LR GT}};
	\end{tikzpicture}
	\begin{tikzpicture}	[spy using outlines={green,magnification=\ssmag,size=\ssizz},inner sep=0]
        \node [align=center, img] {\includegraphics[width=\imgWidth]{imgs/main/Ev-REDS/EDI-1x.png}};         \spy on \smallboxloc in node [left] at \largeboxloc;
        \node [anchor=west,font=\fontsize{8}{8}\selectfont] at \scc {\textcolor{white}{\bf  EDI}};
	\end{tikzpicture}
	\begin{tikzpicture}	[spy using outlines={green,magnification=\ssmag,size=\ssizz},inner sep=0]
        \node [align=center, img] {\includegraphics[width=\imgWidth]{imgs/main/Ev-REDS/eSL-1x.png}};         \spy on \smallboxloc in node [left] at \largeboxloc;
        \node [anchor=west,font=\fontsize{8}{8}\selectfont] at \scc {\textcolor{white}{\bf  eSL-Net}};
	\end{tikzpicture}
	\begin{tikzpicture}	[spy using outlines={green,magnification=\ssmag,size=\ssizz},inner sep=0]
        \node [align=center, img] {\includegraphics[width=\imgWidth]{imgs/main/Ev-REDS/RED-1x.png}};         \spy on \smallboxloc in node [left] at \largeboxloc;
        \node [anchor=west,font=\fontsize{8}{8}\selectfont] at \scc {\textcolor{white}{\bf  RED}};
	\end{tikzpicture}
	\begin{tikzpicture}	[spy using outlines={green,magnification=\ssmag,size=\ssizz},inner sep=0]
        \node [align=center, img] {\includegraphics[width=\imgWidth]{imgs/main/Ev-REDS/Ours-1x.png}};         \spy on \smallboxloc in node [left] at \largeboxloc;
        \node [anchor=west,font=\fontsize{8}{8}\selectfont] at \scc {\textcolor{white}{\bf  Ours}};
	\end{tikzpicture}
	\\
	\begin{tikzpicture}	[spy using outlines={green,magnification=\ssmag,size=\ssizz},inner sep=0]
        \node [align=center, img] {\includegraphics[width=\imgWidth]{imgs/main/Ev-REDS/Blur-4x-full.png}};         \spy on \smallboxloc in node [left] at \largeboxloc;
        \node [anchor=west,font=\fontsize{8}{8}\selectfont] at \scc {\textcolor{white}{\bf HR blur}};
	\end{tikzpicture}
	\begin{tikzpicture}	[spy using outlines={green,magnification=\ssmag,size=\ssizz},inner sep=0]
        \node [align=center, img] {\includegraphics[width=\imgWidth]{imgs/main/Ev-REDS/GT-4x-full.png}};         \spy on \smallboxloc in node [left] at \largeboxloc;
        \node [anchor=west,font=\fontsize{8}{8}\selectfont] at \scc {\textcolor{white}{\bf HR GT}};
	\end{tikzpicture}
	\begin{tikzpicture}	[spy using outlines={green,magnification=\ssmag,size=\ssizz},inner sep=0]
        \node [align=center, img] {\includegraphics[width=\imgWidth]{imgs/main/Ev-REDS/EDI-4x-full.png}};         \spy on \smallboxloc in node [left] at \largeboxloc;
        \node [anchor=west,font=\fontsize{8}{8}\selectfont] at \scc {\textcolor{white}{\bf  EDI+DASR}};
	\end{tikzpicture}
	\begin{tikzpicture}	[spy using outlines={green,magnification=\ssmag,size=\ssizz},inner sep=0]
        \node [align=center, img] {\includegraphics[width=\imgWidth]{imgs/main/Ev-REDS/eSL-4x-full.png}};         \spy on \smallboxloc in node [left] at \largeboxloc;
        \node [anchor=west,font=\fontsize{8}{8}\selectfont] at \scc {\textcolor{white}{\bf \bf  eSL-Net}};
	\end{tikzpicture}
	\begin{tikzpicture}	[spy using outlines={green,magnification=\ssmag,size=\ssizz},inner sep=0]
        \node [align=center, img] {\includegraphics[width=\imgWidth]{imgs/main/Ev-REDS/RED+DASR-4x-full.png}};         \spy on \smallboxloc in node [left] at \largeboxloc;
        \node [anchor=west,font=\fontsize{8}{8}\selectfont] at \scc {\textcolor{white}{\bf \bf  RED+DASR}};
	\end{tikzpicture}
	\begin{tikzpicture}	[spy using outlines={green,magnification=\ssmag,size=\ssizz},inner sep=0]
        \node [align=center, img] {\includegraphics[width=\imgWidth]{imgs/main/Ev-REDS/Ours-4x-full.png}};         \spy on \smallboxloc in node [left] at \largeboxloc;
        \node [anchor=west,font=\fontsize{8}{8}\selectfont] at \scc {\textcolor{white}{\bf \bf  Ours}};
	\end{tikzpicture}

 
	\vspace{-0.75em}
	\caption{ Qualitative comparisons under different spatial scales $\mathcal{R}(B_T,\mathcal{E}_\mathcal{T})=1$ (LR blur, top row) and $\mathcal{R}(B_T,\mathcal{E}_\mathcal{T})=4$ (HR blur, bottom row) on the Ev-REDS dataset. Our results are converted to gray-scale for fair comparisons. 
% 	Details are zoomed in for a better view.
	}
    \vspace{-0.75em}
	\label{fig:ev-reds}
\end{figure*}











%\def\scc{(-1.38,-0.75)}
% \def\boxloc{(-1.65,-0.2)}
% \def\imgWidth{0.162\textwidth} %子图大小

% \begin{figure*}[t]
% 	\centering
% 	\tikzstyle{img} = [rectangle, minimum width=\imgWidth, draw=white]
% % 	\rotatebox[origin=c]{90}{\centering \scriptsize{hahahahhah}}
% 	\begin{tikzpicture}	[inner sep=0]
% 	   % \node [anchor=west,font=\fontsize{6}{6}\selectfont] at \boxloc {\rotatebox{90}{LR frames \& events}};
%         \node [align=center, img] {\includegraphics[width=\imgWidth]{imgs/main/Ev-REDS/Blur-1x.png}};
%         \node [anchor=west,font=\fontsize{8}{8}\selectfont] at \scc {\textcolor{white}{\bf  $1\times$ Blur}};
% 	\end{tikzpicture}
% 	\begin{tikzpicture}	[inner sep=0]
%         \node [align=center, img] {\includegraphics[width=\imgWidth]{imgs/main/Ev-REDS/GT-1x.png}};
%         \node [anchor=west,font=\fontsize{8}{8}\selectfont] at \scc {\textcolor{white}{\bf  GT}};
% 	\end{tikzpicture}
% 	\begin{tikzpicture}	[inner sep=0]
%         \node [align=center, img] {\includegraphics[width=\imgWidth]{imgs/main/Ev-REDS/EDI-1x.png}};
%         \node [anchor=west,font=\fontsize{8}{8}\selectfont] at \scc {\textcolor{white}{\bf  EDI}};
% 	\end{tikzpicture}
% 	\begin{tikzpicture}	[inner sep=0]
%         \node [align=center, img] {\includegraphics[width=\imgWidth]{imgs/main/Ev-REDS/eSL-1x.png}};
%         \node [anchor=west,font=\fontsize{8}{8}\selectfont] at \scc {\textcolor{white}{\bf  eSL-Net}};
% 	\end{tikzpicture}
% 	\begin{tikzpicture}	[inner sep=0]
%         \node [align=center, img] {\includegraphics[width=\imgWidth]{imgs/main/Ev-REDS/RED-1x.png}};
%         \node [anchor=west,font=\fontsize{8}{8}\selectfont] at \scc {\textcolor{white}{\bf  RED}};
% 	\end{tikzpicture}
% 	\begin{tikzpicture}	[inner sep=0]
%         \node [align=center, img] {\includegraphics[width=\imgWidth]{imgs/main/Ev-REDS/Ours-1x.png}};
%         \node [anchor=west,font=\fontsize{8}{8}\selectfont] at \scc {\textcolor{white}{\bf  Ours}};
% 	\end{tikzpicture}
% 	\\
% 	\begin{tikzpicture}	[inner sep=0]
%         \node [align=center, img] {\includegraphics[width=\imgWidth]{imgs/main/Ev-REDS/Blur-4x.png}};
%         \node [anchor=west,font=\fontsize{8}{8}\selectfont] at \scc {\textcolor{white}{\bf $4\times$ Blur}};
% 	\end{tikzpicture}
% 	\begin{tikzpicture}	[inner sep=0]
%         \node [align=center, img] {\includegraphics[width=\imgWidth]{imgs/main/Ev-REDS/GT-4x.png}};
%         \node [anchor=west,font=\fontsize{8}{8}\selectfont] at \scc {\textcolor{white}{\bf  GT}};
% 	\end{tikzpicture}
% 	\begin{tikzpicture}	[inner sep=0]
%         \node [align=center, img] {\includegraphics[width=\imgWidth]{imgs/main/Ev-REDS/EDI-4x.png}};
%         \node [anchor=west,font=\fontsize{8}{8}\selectfont] at \scc {\textcolor{white}{\bf  EDI+DASR}};
% 	\end{tikzpicture}
% 	\begin{tikzpicture}	[inner sep=0]
%         \node [align=center, img] {\includegraphics[width=\imgWidth]{imgs/main/Ev-REDS/eSL-4x.png}};
%         \node [anchor=west,font=\fontsize{8}{8}\selectfont] at \scc {\textcolor{white}{\bf \bf  eSL-Net}};
% 	\end{tikzpicture}
% 	\begin{tikzpicture}	[inner sep=0]
%         \node [align=center, img] {\includegraphics[width=\imgWidth]{imgs/main/Ev-REDS/RED+DASR-4x.png}};
%         \node [anchor=west,font=\fontsize{8}{8}\selectfont] at \scc {\textcolor{white}{\bf \bf  RED+DASR}};
% 	\end{tikzpicture}
% 	\begin{tikzpicture}	[inner sep=0]
%         \node [align=center, img] {\includegraphics[width=\imgWidth]{imgs/main/Ev-REDS/Ours-4x.png}};
%         \node [anchor=west,font=\fontsize{8}{8}\selectfont] at \scc {\textcolor{white}{\bf \bf  Ours}};
% 	\end{tikzpicture}
	
% 	\caption{ Qualitative comparisons on the Ev-REDS dataset under $\mathcal{R}(B_T,\mathcal{E}_\mathcal{T})=1$ ($1\times$ blur, top row) and $\mathcal{R}(B_T,\mathcal{E}_\mathcal{T})=4$ ($4\times$ blur, bottom row). Reconstruction details are shown in the case of $4\times$ blur. Our results are converted to gray-scale for fair comparison. 
% 	}
% 	\label{fig:ev-reds}
% \end{figure*}

==> figs/main/fig-HS-ERGB.tex <==
\def\scc{(-1.38,-1.5)}
\def\boxloc{(-1.65,-0.2)}
\def\imgWidth{0.162\textwidth} %子图大小

\def\ssizz{1cm} %框大小
\def\ssmag{3}
% \def\smallboxloc{(1.23,0.03)} % 绿色小方框位置
\def\smallboxloc{(1.25,-0.4)} % 绿色小方框位置
\def\largeboxloc{(-0.35, 1.13)} % 绿色大方框位置

\begin{figure*}[t]
	\centering
	\tikzstyle{img} = [rectangle, minimum width=\imgWidth, draw=white]
% 	\rotatebox[origin=c]{90}{\centering \scriptsize{hahahahhah}}
	\begin{tikzpicture}	[spy using outlines={green,magnification=\ssmag,size=\ssizz},inner sep=0]
        \node [align=center, img] {\includegraphics[width=\imgWidth]{imgs/main/HS-ERGB/Blur-7blur-1x.png}};         \spy on \smallboxloc in node [left] at \largeboxloc;
        \node [anchor=west,font=\fontsize{8}{8}\selectfont] at \scc {\textcolor{white}{\bf Normal blur}};
	\end{tikzpicture}
	\begin{tikzpicture}	[spy using outlines={green,magnification=\ssmag,size=\ssizz},inner sep=0]
        \node [align=center, img] {\includegraphics[width=\imgWidth]{imgs/main/HS-ERGB/GT-1x.png}};         \spy on \smallboxloc in node [left] at \largeboxloc;
        \node [anchor=west,font=\fontsize{8}{8}\selectfont] at \scc {\textcolor{white}{\bf GT}};
	\end{tikzpicture}
	\begin{tikzpicture}	[spy using outlines={green,magnification=\ssmag,size=\ssizz},inner sep=0]
        \node [align=center, img] {\includegraphics[width=\imgWidth]{imgs/main/HS-ERGB/LEVS-7blur-1x.png}};         \spy on \smallboxloc in node [left] at \largeboxloc;
        \node [anchor=west,font=\fontsize{8}{8}\selectfont] at \scc {\textcolor{white}{\bf LEVS}};
	\end{tikzpicture}
	\begin{tikzpicture}	[spy using outlines={green,magnification=\ssmag,size=\ssizz},inner sep=0]
        \node [align=center, img] {\includegraphics[width=\imgWidth]{imgs/main/HS-ERGB/Motion-ETR-7blur-1x.png}};         \spy on \smallboxloc in node [left] at \largeboxloc;
        \node [anchor=west,font=\fontsize{8}{8}\selectfont] at \scc {\textcolor{white}{\bf Motion-ETR}};
	\end{tikzpicture}
	\begin{tikzpicture}	[spy using outlines={green,magnification=\ssmag,size=\ssizz},inner sep=0]
        \node [align=center, img] {\includegraphics[width=\imgWidth]{imgs/main/HS-ERGB/EVDI-7blur-1x.png}};         \spy on \smallboxloc in node [left] at \largeboxloc;
        \node [anchor=west,font=\fontsize{8}{8}\selectfont] at \scc {\textcolor{white}{\bf EVDI}};
	\end{tikzpicture}
	\begin{tikzpicture}	[spy using outlines={green,magnification=\ssmag,size=\ssizz},inner sep=0]
        \node [align=center, img] {\includegraphics[width=\imgWidth]{imgs/main/HS-ERGB/Ours-7blur-1x.png}};         \spy on \smallboxloc in node [left] at \largeboxloc;
        \node [anchor=west,font=\fontsize{8}{8}\selectfont] at \scc {\textcolor{white}{\bf Ours}};
	\end{tikzpicture}
	\\
	\begin{tikzpicture}	[spy using outlines={green,magnification=\ssmag,size=\ssizz},inner sep=0]
        \node [align=center, img] {\includegraphics[width=\imgWidth]{imgs/main/HS-ERGB/Blur-13blur-1x.png}};         \spy on \smallboxloc in node [left] at \largeboxloc;
        \node [anchor=west,font=\fontsize{8}{8}\selectfont] at \scc {\textcolor{white}{\bf Large blur}};
	\end{tikzpicture}
	\begin{tikzpicture}	[spy using outlines={green,magnification=\ssmag,size=\ssizz},inner sep=0]
        \node [align=center, img] {\includegraphics[width=\imgWidth]{imgs/main/HS-ERGB/GT-1x.png}};         \spy on \smallboxloc in node [left] at \largeboxloc;
        \node [anchor=west,font=\fontsize{8}{8}\selectfont] at \scc {\textcolor{white}{\bf GT}};
	\end{tikzpicture}
	\begin{tikzpicture}	[spy using outlines={green,magnification=\ssmag,size=\ssizz},inner sep=0]
        \node [align=center, img] {\includegraphics[width=\imgWidth]{imgs/main/HS-ERGB/LEVS-13blur-1x.png}};         \spy on \smallboxloc in node [left] at \largeboxloc;
        \node [anchor=west,font=\fontsize{8}{8}\selectfont] at \scc {\textcolor{white}{\bf LEVS}};
	\end{tikzpicture}
	\begin{tikzpicture}	[spy using outlines={green,magnification=\ssmag,size=\ssizz},inner sep=0]
        \node [align=center, img] {\includegraphics[width=\imgWidth]{imgs/main/HS-ERGB/Motion-ETR-13blur-1x.png}};         \spy on \smallboxloc in node [left] at \largeboxloc;
        \node [anchor=west,font=\fontsize{8}{8}\selectfont] at \scc {\textcolor{white}{\bf Motion-ETR}};
	\end{tikzpicture}
	\begin{tikzpicture}	[spy using outlines={green,magnification=\ssmag,size=\ssizz},inner sep=0]
        \node [align=center, img] {\includegraphics[width=\imgWidth]{imgs/main/HS-ERGB/EVDI-13blur-1x.png}};         \spy on \smallboxloc in node [left] at \largeboxloc;
        \node [anchor=west,font=\fontsize{8}{8}\selectfont] at \scc {\textcolor{white}{\bf EVDI}};
	\end{tikzpicture}
	\begin{tikzpicture}	[spy using outlines={green,magnification=\ssmag,size=\ssizz},inner sep=0]
        \node [align=center, img] {\includegraphics[width=\imgWidth]{imgs/main/HS-ERGB/Ours-13blur-1x.png}};         \spy on \smallboxloc in node [left] at \largeboxloc;
        \node [anchor=west,font=\fontsize{8}{8}\selectfont] at \scc {\textcolor{white}{\bf Ours}};
	\end{tikzpicture}
 
	\vspace{-0.75em}
	\caption{ Qualitative comparisons under normal blur (top row) and large blur (bottom row) on the HS-ERGB dataset.
	}
    \vspace{-0.75em}
	\label{fig:hs-ergb}
\end{figure*}





% \def\scc{(-1.38,-1.5)}
% \def\boxloc{(-1.65,-0.2)}
% \def\imgWidth{0.162\textwidth} %子图大小

% \begin{figure*}[t]
% 	\centering
% 	\tikzstyle{img} = [rectangle, minimum width=\imgWidth, draw=white]
% % 	\rotatebox[origin=c]{90}{\centering \scriptsize{hahahahhah}}
% 	\begin{tikzpicture}	[inner sep=0]
%         \node [align=center, img] {\includegraphics[width=\imgWidth]{imgs/main/HS-ERGB/Blur-7blur-1x.png}};
%         \node [anchor=west,font=\fontsize{8}{8}\selectfont] at \scc {\textcolor{white}{\bf Normal blur}};
% 	\end{tikzpicture}
% 	\begin{tikzpicture}	[inner sep=0]
%         \node [align=center, img] {\includegraphics[width=\imgWidth]{imgs/main/HS-ERGB/GT-1x.png}};
%         \node [anchor=west,font=\fontsize{8}{8}\selectfont] at \scc {\textcolor{white}{\bf GT}};
% 	\end{tikzpicture}
% 	\begin{tikzpicture}	[inner sep=0]
%         \node [align=center, img] {\includegraphics[width=\imgWidth]{imgs/main/HS-ERGB/LEVS-7blur-1x.png}};
%         \node [anchor=west,font=\fontsize{8}{8}\selectfont] at \scc {\textcolor{white}{\bf LEVS}};
% 	\end{tikzpicture}
% 	\begin{tikzpicture}	[inner sep=0]
%         \node [align=center, img] {\includegraphics[width=\imgWidth]{imgs/main/HS-ERGB/Motion-ETR-7blur-1x.png}};
%         \node [anchor=west,font=\fontsize{8}{8}\selectfont] at \scc {\textcolor{white}{\bf Motion-ETR}};
% 	\end{tikzpicture}
% 	\begin{tikzpicture}	[inner sep=0]
%         \node [align=center, img] {\includegraphics[width=\imgWidth]{imgs/main/HS-ERGB/EVDI-7blur-1x.png}};
%         \node [anchor=west,font=\fontsize{8}{8}\selectfont] at \scc {\textcolor{white}{\bf EVDI}};
% 	\end{tikzpicture}
% 	\begin{tikzpicture}	[inner sep=0]
%         \node [align=center, img] {\includegraphics[width=\imgWidth]{imgs/main/HS-ERGB/Ours-7blur-1x.png}};
%         \node [anchor=west,font=\fontsize{8}{8}\selectfont] at \scc {\textcolor{white}{\bf Ours}};
% 	\end{tikzpicture}
% 	\\
% 	\begin{tikzpicture}	[inner sep=0]
%         \node [align=center, img] {\includegraphics[width=\imgWidth]{imgs/main/HS-ERGB/Blur-13blur-1x.png}};
%         \node [anchor=west,font=\fontsize{8}{8}\selectfont] at \scc {\textcolor{white}{\bf Large blur}};
% 	\end{tikzpicture}
% 	\begin{tikzpicture}	[inner sep=0]
%         \node [align=center, img] {\includegraphics[width=\imgWidth]{imgs/main/HS-ERGB/GT-1x.png}};
%         \node [anchor=west,font=\fontsize{8}{8}\selectfont] at \scc {\textcolor{white}{\bf GT}};
% 	\end{tikzpicture}
% 	\begin{tikzpicture}	[inner sep=0]
%         \node [align=center, img] {\includegraphics[width=\imgWidth]{imgs/main/HS-ERGB/LEVS-13blur-1x.png}};
%         \node [anchor=west,font=\fontsize{8}{8}\selectfont] at \scc {\textcolor{white}{\bf LEVS}};
% 	\end{tikzpicture}
% 	\begin{tikzpicture}	[inner sep=0]
%         \node [align=center, img] {\includegraphics[width=\imgWidth]{imgs/main/HS-ERGB/Motion-ETR-13blur-1x.png}};
%         \node [anchor=west,font=\fontsize{8}{8}\selectfont] at \scc {\textcolor{white}{\bf Motion-ETR}};
% 	\end{tikzpicture}
% 	\begin{tikzpicture}	[inner sep=0]
%         \node [align=center, img] {\includegraphics[width=\imgWidth]{imgs/main/HS-ERGB/EVDI-13blur-1x.png}};
%         \node [anchor=west,font=\fontsize{8}{8}\selectfont] at \scc {\textcolor{white}{\bf EVDI}};
% 	\end{tikzpicture}
% 	\begin{tikzpicture}	[inner sep=0]
%         \node [align=center, img] {\includegraphics[width=\imgWidth]{imgs/main/HS-ERGB/Ours-13blur-1x.png}};
%         \node [anchor=west,font=\fontsize{8}{8}\selectfont] at \scc {\textcolor{white}{\bf Ours}};
% 	\end{tikzpicture}
	
% 	\caption{ Qualitative comparisons on the HS-ERGB dataset under normal blur (top row) and large blur (bottom row).
% 	}
% 	\label{fig:hs-ergb}
% \end{figure*}

==> figs/main/fig-MS-RBD.tex <==
\def\scc{(-1.65,-0.96)}
\def\imgWidth{0.195\textwidth} %子图大小

\def\ssizz{1cm} %框大小
\def\ssmag{3}
\def\smallboxloc{(0.4,-0.15)} % 绿色小方框位置
\def\largeboxloc{(-0.65, 0.59)} % 绿色大方框位置

% \def\smallboxlocout{(0.75,-0.15)} % 绿色小方框位置
\def\smallboxlocout{(0.75,-0.2)} % 绿色小方框位置

% bag
% \def\ssizz{1cm} %框大小
% \def\ssmag{3}
% \def\smallboxloc{(1.1,0.32)} % 绿色小方框位置
% \def\largeboxloc{(1.65, -0.59)} % 绿色大方框位置

\begin{figure*}[t]
	\centering
	\tikzstyle{img} = [rectangle, minimum width=\imgWidth, draw=white]
	\begin{tikzpicture}	[spy using outlines={green,magnification=\ssmag,size=\ssizz},inner sep=0]
        \node [align=center, img] {\includegraphics[width=\imgWidth]{imgs/main/MS-RBD/in/Blur-1x.png}};
        \spy on \smallboxloc in node [left] at \largeboxloc;
        \node [anchor=west,font=\fontsize{8}{8}\selectfont] at \scc {\textcolor{white}{\bf Blur}};
	\end{tikzpicture}
	\begin{tikzpicture}	[spy using outlines={green,magnification=\ssmag,size=\ssizz},inner sep=0]
        \node [align=center, img] {\includegraphics[width=\imgWidth]{imgs/main/MS-RBD/in/LEVS-1x.png}};
        \spy on \smallboxloc in node [left] at \largeboxloc;
        \node [anchor=west,font=\fontsize{8}{8}\selectfont] at \scc {\textcolor{white}{\bf LEVS}};
	\end{tikzpicture}
	\begin{tikzpicture}	[spy using outlines={green,magnification=\ssmag,size=\ssizz},inner sep=0]
        \node [align=center, img] {\includegraphics[width=\imgWidth]{imgs/main/MS-RBD/in/Motion-ETR-1x.png}};
        \spy on \smallboxloc in node [left] at \largeboxloc;
        \node [anchor=west,font=\fontsize{8}{8}\selectfont] at \scc {\textcolor{white}{\bf Motion-ETR}};
	\end{tikzpicture}
	\begin{tikzpicture}	[spy using outlines={green,magnification=\ssmag,size=\ssizz},inner sep=0]
        \node [align=center, img] {\includegraphics[width=\imgWidth]{imgs/main/MS-RBD/in/EVDI+DASR-1x.png}};
        \spy on \smallboxloc in node [left] at \largeboxloc;
        \node [anchor=west,font=\fontsize{8}{8}\selectfont] at \scc {\textcolor{white}{\bf EVDI+DASR}};
	\end{tikzpicture}
	\begin{tikzpicture}	[spy using outlines={green,magnification=\ssmag,size=\ssizz},inner sep=0]
        \node [align=center, img] {\includegraphics[width=\imgWidth]{imgs/main/MS-RBD/in/Ours-1x.png}};
        \spy on \smallboxloc in node [left] at \largeboxloc;
        \node [anchor=west,font=\fontsize{8}{8}\selectfont] at \scc {\textcolor{white}{\bf Ours}};
	\end{tikzpicture}
\\
\begin{tikzpicture}	[spy using outlines={green,magnification=\ssmag,size=\ssizz},inner sep=0]
        \node [align=center, img] {\includegraphics[width=\imgWidth]{imgs/main/MS-RBD/out/Blur-1x.png}};
        \spy on \smallboxlocout in node [left] at \largeboxloc;
        \node [anchor=west,font=\fontsize{8}{8}\selectfont] at \scc {\textcolor{white}{\bf Blur}};
	\end{tikzpicture}
	\begin{tikzpicture}	[spy using outlines={green,magnification=\ssmag,size=\ssizz},inner sep=0]
        \node [align=center, img] {\includegraphics[width=\imgWidth]{imgs/main/MS-RBD/out/LEVS-1x.png}};
        \spy on \smallboxlocout in node [left] at \largeboxloc;
        \node [anchor=west,font=\fontsize{8}{8}\selectfont] at \scc {\textcolor{white}{\bf LEVS}};
	\end{tikzpicture}
	\begin{tikzpicture}	[spy using outlines={green,magnification=\ssmag,size=\ssizz},inner sep=0]
        \node [align=center, img] {\includegraphics[width=\imgWidth]{imgs/main/MS-RBD/out/Motion-ETR-1x.png}};
        \spy on \smallboxlocout in node [left] at \largeboxloc;
        \node [anchor=west,font=\fontsize{8}{8}\selectfont] at \scc {\textcolor{white}{\bf Motion-ETR}};
	\end{tikzpicture}
	\begin{tikzpicture}	[spy using outlines={green,magnification=\ssmag,size=\ssizz},inner sep=0]
        \node [align=center, img] {\includegraphics[width=\imgWidth]{imgs/main/MS-RBD/out/EVDI+DASR-1x.png}};
        \spy on \smallboxlocout in node [left] at \largeboxloc;
        \node [anchor=west,font=\fontsize{8}{8}\selectfont] at \scc {\textcolor{white}{\bf EVDI+DASR}};
	\end{tikzpicture}
	\begin{tikzpicture}	[spy using outlines={green,magnification=\ssmag,size=\ssizz},inner sep=0]
        \node [align=center, img] {\includegraphics[width=\imgWidth]{imgs/main/MS-RBD/out/Ours-1x.png}};
        \spy on \smallboxlocout in node [left] at \largeboxloc;
        \node [anchor=west,font=\fontsize{8}{8}\selectfont] at \scc {\textcolor{white}{\bf Ours}};
	\end{tikzpicture}

	\vspace{-0.75em}
	\caption{ Qualitative comparisons under real-world HR frames and LR events on our MS-RBD. 
 % Details are zoomed in for a better view.
	}
        \vspace{-0.75em}
	\label{fig:ms-rbd}
\end{figure*}


%%% original version ====================
% \def\scc{(-1.65,-0.96)}
% \def\imgWidth{0.195\textwidth} %子图大小

% \def\ssizz{1cm} %框大小
% \def\ssmag{3}
% \def\smallboxloc{(1.02,0)} % 绿色小方框位置
% \def\largeboxloc{(-0.65, 0.59)} % 绿色大方框位置

% % \def\smallboxlocout{(0.75,-0.15)} % 绿色小方框位置
% \def\smallboxlocout{(0.75,-0.2)} % 绿色小方框位置

% % bag
% % \def\ssizz{1cm} %框大小
% % \def\ssmag{3}
% % \def\smallboxloc{(1.1,0.32)} % 绿色小方框位置
% % \def\largeboxloc{(1.65, -0.59)} % 绿色大方框位置

% \begin{figure*}[t]
% 	\centering
% 	\tikzstyle{img} = [rectangle, minimum width=\imgWidth, draw=white]
% 	\begin{tikzpicture}	[spy using outlines={green,magnification=\ssmag,size=\ssizz},inner sep=0]
%         \node [align=center, img] {\includegraphics[width=\imgWidth]{imgs/main/MS-RBD/Blur-1x.png}};
%         \spy on \smallboxloc in node [left] at \largeboxloc;
%         \node [anchor=west,font=\fontsize{8}{8}\selectfont] at \scc {\textcolor{white}{\bf Blur}};
% 	\end{tikzpicture}
% 	\begin{tikzpicture}	[spy using outlines={green,magnification=\ssmag,size=\ssizz},inner sep=0]
%         \node [align=center, img] {\includegraphics[width=\imgWidth]{imgs/main/MS-RBD/LEVS-1x.png}};
%         \spy on \smallboxloc in node [left] at \largeboxloc;
%         \node [anchor=west,font=\fontsize{8}{8}\selectfont] at \scc {\textcolor{white}{\bf LEVS}};
% 	\end{tikzpicture}
% 	\begin{tikzpicture}	[spy using outlines={green,magnification=\ssmag,size=\ssizz},inner sep=0]
%         \node [align=center, img] {\includegraphics[width=\imgWidth]{imgs/main/MS-RBD/Motion-ETR-1x.png}};
%         \spy on \smallboxloc in node [left] at \largeboxloc;
%         \node [anchor=west,font=\fontsize{8}{8}\selectfont] at \scc {\textcolor{white}{\bf Motion-ETR}};
% 	\end{tikzpicture}
% 	\begin{tikzpicture}	[spy using outlines={green,magnification=\ssmag,size=\ssizz},inner sep=0]
%         \node [align=center, img] {\includegraphics[width=\imgWidth]{imgs/main/MS-RBD/EVDI+DASR-1x.png}};
%         \spy on \smallboxloc in node [left] at \largeboxloc;
%         \node [anchor=west,font=\fontsize{8}{8}\selectfont] at \scc {\textcolor{white}{\bf EVDI+DASR}};
% 	\end{tikzpicture}
% 	\begin{tikzpicture}	[spy using outlines={green,magnification=\ssmag,size=\ssizz},inner sep=0]
%         \node [align=center, img] {\includegraphics[width=\imgWidth]{imgs/main/MS-RBD/Ours-1x.png}};
%         \spy on \smallboxloc in node [left] at \largeboxloc;
%         \node [anchor=west,font=\fontsize{8}{8}\selectfont] at \scc {\textcolor{white}{\bf Ours}};
% 	\end{tikzpicture}
% \\
% \begin{tikzpicture}	[spy using outlines={green,magnification=\ssmag,size=\ssizz},inner sep=0]
%         \node [align=center, img] {\includegraphics[width=\imgWidth]{imgs/main/MS-RBD/out/Blur-1x.png}};
%         \spy on \smallboxlocout in node [left] at \largeboxloc;
%         \node [anchor=west,font=\fontsize{8}{8}\selectfont] at \scc {\textcolor{white}{\bf Blur}};
% 	\end{tikzpicture}
% 	\begin{tikzpicture}	[spy using outlines={green,magnification=\ssmag,size=\ssizz},inner sep=0]
%         \node [align=center, img] {\includegraphics[width=\imgWidth]{imgs/main/MS-RBD/out/LEVS-1x.png}};
%         \spy on \smallboxlocout in node [left] at \largeboxloc;
%         \node [anchor=west,font=\fontsize{8}{8}\selectfont] at \scc {\textcolor{white}{\bf LEVS}};
% 	\end{tikzpicture}
% 	\begin{tikzpicture}	[spy using outlines={green,magnification=\ssmag,size=\ssizz},inner sep=0]
%         \node [align=center, img] {\includegraphics[width=\imgWidth]{imgs/main/MS-RBD/out/Motion-ETR-1x.png}};
%         \spy on \smallboxlocout in node [left] at \largeboxloc;
%         \node [anchor=west,font=\fontsize{8}{8}\selectfont] at \scc {\textcolor{white}{\bf Motion-ETR}};
% 	\end{tikzpicture}
% 	\begin{tikzpicture}	[spy using outlines={green,magnification=\ssmag,size=\ssizz},inner sep=0]
%         \node [align=center, img] {\includegraphics[width=\imgWidth]{imgs/main/MS-RBD/out/EVDI+DASR-1x.png}};
%         \spy on \smallboxlocout in node [left] at \largeboxloc;
%         \node [anchor=west,font=\fontsize{8}{8}\selectfont] at \scc {\textcolor{white}{\bf EVDI+DASR}};
% 	\end{tikzpicture}
% 	\begin{tikzpicture}	[spy using outlines={green,magnification=\ssmag,size=\ssizz},inner sep=0]
%         \node [align=center, img] {\includegraphics[width=\imgWidth]{imgs/main/MS-RBD/out/Ours-1x.png}};
%         \spy on \smallboxlocout in node [left] at \largeboxloc;
%         \node [anchor=west,font=\fontsize{8}{8}\selectfont] at \scc {\textcolor{white}{\bf Ours}};
% 	\end{tikzpicture}

% 	\vspace{-0.75em}
% 	\caption{ Qualitative comparisons under real-world HR frames and LR events on our MS-RBD. 
%  % Details are zoomed in for a better view.
% 	}
%         \vspace{-0.75em}
% 	\label{fig:ms-rbd}
% \end{figure*}

==> figs/main/fig-insight.tex <==
\def\scc{(-1.3,-0.72)}
\def\imgWidth{0.32\linewidth} %子图大小

\begin{figure}[t]
	\centering
	\tikzstyle{img} = [rectangle, minimum width=\imgWidth, draw=white]
	\begin{tikzpicture}	[inner sep=0]
        \node [align=center, img] {\includegraphics[width=\imgWidth]{imgs/main/insight/Blur-1x.png}};
        \node [anchor=west,font=\fontsize{8}{8}\selectfont] at \scc {\textcolor{white}{\bf Blur}};
	\end{tikzpicture}
	\begin{tikzpicture}	[inner sep=0]
        \node [align=center, img] {\includegraphics[width=\imgWidth]{imgs/main/insight/Model1-1x.png}};
        \node [anchor=west,font=\fontsize{8}{8}\selectfont] at \scc {\textcolor{white}{\bf  Result}};
	\end{tikzpicture}
	\begin{tikzpicture}	[inner sep=0]
        \node [align=center, img] {\includegraphics[width=\imgWidth]{imgs/main/insight/GT-1x.png}};
        \node [anchor=west,font=\fontsize{8}{8}\selectfont] at \scc {\textcolor{white}{\bf  GT}};
	\end{tikzpicture}
        \vspace{-0.5em}
	\caption{ Results of our model trained only with blur conversion, \ie, $\mathcal{L}_{BC}$ in Eq.~\eqref{eq:loss_bc}, which achieves a coarse deblurring performance without using ground-truth images for supervision. }
        \vspace{-1.5em}
	\label{fig:insight}
\end{figure}



% \begin{tikzpicture}[spy using outlines={green,magnification=\ssmag,size=\ssizz},inner sep=0]
%             \node [align=center, img] {\includegraphics[width=\imgWidth]{Figs/Res-Deblur/leftB.png}};
%             % \spy on \ssxxsone in node [left] at \ssyysone;
%             \node [anchor=west] at \scc {\textcolor{white}{\bf Left blurry}};
%     	\end{tikzpicture}


% \begin{figure}[t]
% 	\centering
% 	\begin{subfigure}{0.32\linewidth}
% 	\centering
% 		\includegraphics[width=\linewidth]{imgs/main/insight/Blur-1x.png}
% 	\end{subfigure}
% 	\begin{subfigure}{0.32\linewidth}
% 	\centering
% 		\includegraphics[width=\linewidth]{imgs/main/insight/Model1-1x.png}
% 	\end{subfigure}
% 	\begin{subfigure}{0.32\linewidth}
% 	\centering
% 		\includegraphics[width=\linewidth]{imgs/main/insight/GT-1x.png}
% 	\end{subfigure}
% 	\caption{ TODO }
% 	\label{fig:insight}
% \end{figure}


==> figs/rebuttal/fig-reRED.tex <==
\def\scc{(-0.95,-0.55)}
\def\imgWidth{0.24\linewidth} %子图大小

\def\ssizz{0.75cm} %框大小
\def\ssmag{3}
\def\smallboxloc{(-0.45,0.22)} % 绿色小方框位置
\def\largeboxloc{(0.95, 0.3)} % 绿色大方框位置

% \begin{tikzpicture}	[spy using outlines={green,magnification=\ssmag,size=\ssizz},inner sep=0]
%         \node [align=center, img] {\includegraphics[width=\imgWidth]{imgs/main/Ev-REDS/GT-1x.png}};         \spy on \smallboxloc in node [left] at \largeboxloc;
%         \node [anchor=west,font=\fontsize{8}{8}\selectfont] at \scc {\textcolor{white}{\bf LR GT}};
% 	\end{tikzpicture}

\begin{figure}[ht]
\vspace{-1em}
	\centering
	\tikzstyle{img} = [rectangle, minimum width=\imgWidth, draw=white]
 \begin{tikzpicture}	[spy using outlines={green,magnification=\ssmag,size=\ssizz},inner sep=0]
        \node [align=center, img] {\includegraphics[width=\imgWidth,trim={50px 0px 50px 0px},clip]{imgs/rebuttal/blur.png}};  \spy on \smallboxloc in node [left] at \largeboxloc;
        \node [anchor=west,font=\fontsize{8}{8}\selectfont] at \scc {\textcolor{white}{\bf Blur}};
	\end{tikzpicture}
	\begin{tikzpicture}		[spy using outlines={green,magnification=\ssmag,size=\ssizz},inner sep=0]
        \node [align=center, img] {\includegraphics[width=\imgWidth,trim={50px 0px 50px 0px},clip]{imgs/rebuttal/red.png}}; \spy on \smallboxloc in node [left] at \largeboxloc;
        \node [anchor=west,font=\fontsize{8}{8}\selectfont] at \scc {\textcolor{white}{\bf  RED*}};
	\end{tikzpicture}
     \begin{tikzpicture}	[spy using outlines={green,magnification=\ssmag,size=\ssizz},inner sep=0]
        \node [align=center, img] {\includegraphics[width=\imgWidth,trim={50px 0px 50px 0px},clip]{imgs/rebuttal/ours-LBC.png}}; \spy on \smallboxloc in node [left] at \largeboxloc;
        \node [anchor=west,font=\fontsize{8}{8}\selectfont] at \scc {\textcolor{white}{\bf  GEM*}};
	\end{tikzpicture}
	\begin{tikzpicture}	[spy using outlines={green,magnification=\ssmag,size=\ssizz},inner sep=0]
        \node [align=center, img] {\includegraphics[width=\imgWidth,trim={50px 0px 50px 0px},clip]{imgs/rebuttal/ours.png}}; \spy on \smallboxloc in node [left] at \largeboxloc;
        \node [anchor=west,font=\fontsize{8}{8}\selectfont] at \scc {\textcolor{white}{\bf  GEM}};
	\end{tikzpicture}
        \vspace{-2em}
	\caption{ Qualitative results. * denotes models re-trained by $\mathcal{L}_{BC}$.}
        \vspace{-1em}
	\label{fig:rebuttal-reRED}
\end{figure}


==> tabs/rebuttal/tab-LSG.tex <==
\begin{table}[ht]
\centering
% \small
\scriptsize
\vspace{-1.5em}
% \renewcommand{\arraystretch}{1.1}
\caption{Results of models with and without $\mathcal{L}_{SG}$ under $\mathcal{R}(B_T,\mathcal{E}_{\mathcal{T}})=1$ (LR) and $\mathcal{R}(B_T,\mathcal{E}_{\mathcal{T}})=4$ (HR) on Ev-REDS.}
\vspace{-1em}
\begin{tabular}{c|cccc|c}
\hline
Model & $\mathcal{L}_{BC}$        & $\mathcal{L}_{SC}$      & $\mathcal{L}_{SG}$       & $\mathcal{L}_{TG}$        &    LR /  HR PSNR           \\ \hline
w/o  $\mathcal{L}_{SG}$  & \checkmark &  \checkmark         &           & \checkmark          & 21.95 / \textbf{24.14} \\
w/  $\mathcal{L}_{SG}$  &  \checkmark & \checkmark & \checkmark & \checkmark  & \textbf{24.08} / 24.07   \\\hline
\end{tabular}
\vspace{-1em}
\label{tab:rebuttal_lsg}
\end{table}


==> tabs/rebuttal/tab-baseline.tex <==
\begin{table}[ht]
\centering
\small
\vspace{-1em}
% \renewcommand{\arraystretch}{1.1}
\caption{Comparison with the video-based baseline composed of EVDI and RealBasicVSR under $\mathcal{R}(B_T,\mathcal{E}_{\mathcal{T}})=4$ on Ev-REDS.}
\vspace{-1em}
\begin{tabular}{l|c}
\hline
Method            & PSNR / SSIM             \\ \hline
EVDI+RealBasicVSR & 23.33 / 0.6441          \\
GEM (Ours)        & \textbf{24.07 / 0.6719} \\ \hline
\end{tabular}
\vspace{-1em}
\label{tab:rebuttal-baseline}
\end{table}


==> tabs/rebuttal/tab-eventup.tex <==
\begin{table}[ht]
\centering
% \small
\scriptsize
% \renewcommand{\arraystretch}{1.1}
\vspace{-1em}
\caption{Comparison of event up-sampling and image down-sampling in $\mathcal{L}_{SG}$ on Ev-REDS dataset. Metrics are PSNR / SSIM.}
\vspace{-1em}
\begin{tabular}{l|cc}
\hline
Augmentation in $\mathcal{L}_{SG}$  &  $\mathcal{R}(B_T,\mathcal{E}_{\mathcal{T}})=1$           &  $\mathcal{R}(B_T,\mathcal{E}_{\mathcal{T}})=4$            \\ \hline
Event up-sampling   & 22.12 / 0.7155 & 23.93 / 0.6643 \\
Image down-sampling & \textbf{24.08} / \textbf{0.7898} &\textbf{24.07} / \textbf{0.6719} \\ \hline
\end{tabular}
\vspace{-1em}
\label{tab:rebuttal-evup}
\end{table}


==> tabs/rebuttal/tab-interp.tex <==
\begin{table}[ht]
\centering
\scriptsize
% \renewcommand{\arraystretch}{1.1}
\vspace{-1em}
\caption{Comparison of bicubic interpolation and MSFF in GEM on the Ev-REDS dataset, where the metrics are PSNR / SSIM.}
\vspace{-1em}
\begin{tabular}{l|cc}
\hline
Method  &  $\mathcal{R}(B_T,\mathcal{E}_{\mathcal{T}})=1$           &  $\mathcal{R}(B_T,\mathcal{E}_{\mathcal{T}})=4$            \\ \hline
Bicubic   & 22.37 / 0.7406 & 23.71 / 0.6495 \\
MSFF & \textbf{24.08} / \textbf{0.7898} &\textbf{24.07} / \textbf{0.6719} \\ \hline
\end{tabular}
\vspace{-1em}
\label{tab:rebuttal-interp}
\end{table}

